The time at the subplanckian scale

With the theory of special relativity, time has been linked with space into a four-dimensional space-time from which a basic question must be asked: can space be really transformed into time and vice-versa? The response is affirmative if time has the same structural topological structure as space at the subplanckian quantum level in such a way that a discrete structural quantum time constitutes the time part of the space-time internal vacuum of every elementary particle. It has thus been shown that a quantum time, quantized algebraically according to a lattice of time quanta, really exists and is emergent in the sense that time quanta can be transformed into space quanta and vice-versa. Furthermore,this quantum time, only relevant at the subplanckian scale, is proved to be in one-to-one correspondence with the absolute and relative clock times.

==> cmds.tex <==
\oddsidemargin 0cm
\evensidemargin -12pt
\topmargin -27pt
\textheight 635pt
\textwidth 460pt
\def\baselinestretch{1.2}
\renewcommand{\arraystretch}{1.5}


%definition de leadsto : dans LATEX FONTS
%\def\simarrow{{\scriptstyle{\sim}}\hspace{0.8pt}\mathrel{\raise
%-1.5mm\hbox{$\vec {}\;$}} } 
%\def\leadsto{\mathrel\simarrow}
\def\simarrow{\mathrel{\raise -0.5mm\hbox{$\sim$}}\hspace{-1.8mm}{\rightarrow} } 
\def\rto{\mathrel{\simarrow}}
\def\bsimarrow{\leftarrow\hspace{-0.7mm}\mathrel{\raise -0.5mm\hbox{$\backsim$}} } 
\def\lto{\mathrel{\bsimarrow}}

\newcommand{\fguil}[1]{\guillemotleft~{#1}~\guillemotright}

%     New commands MVC + macros CORE

\newcommand{\tim}[1]{\;\; \mbox{#1} \;\;}

\def\bt{\begin{tabular}}
\def\te{\end{tabular}}

\def\Abstract{\small
\begin{center}
{\bf Abstract\vspace{-.5em}\vspace{0pt}}
\end{center}
\quotation
}
\def\endAbstract{\endquotation}

\def\resume{  \small
\begin{center}
{\bf R\'esum\'e\vspace{-.5em}\vspace{0pt}}
\end{center}
\quotation}
\def\endresume{\endquotation}

\def\lettrine#1#2#3{\noindent\hangindent#1\hangafter-#2
\hskip-#1\smash{\hbox to #1{#3\hfill}}\ignorespaces}

\newcommand{\To}[1]{\mathop{\to}\limits_{#1}}

\def\tog{\renewcommand{\arraystretch}{0.6}
\begin{array}[t]{c}\to\\ >\end{array}}

\def\tol{\renewcommand{\arraystretch}{0.6}
\begin{array}[t]{c}\to\\ <\end{array}}

\def\tog{\renewcommand{\arraystretch}{0.6}
\begin{array}[t]{c}\to\\ >\end{array}}

\def\BM{\begin{pmatrix}}
\def\EM{\end{pmatrix}}


\newcommand{\ms}{\;\;\;\;}

\def\pt{\mathrel{\scriptstyle \bullet}}

\def\txt{\textstyle}
\def\ds{\displaystyle}


\def\cad{c'est-\`{a}-dire\ }

\def\df{\buildrel\hbox{\scriptsize d\'{e}f}\over =}
\def\equivdf{\buildrel\hbox{\scriptsize d\'{e}f}\over \equiv}
\def\nota{\buildrel\hbox{\scriptsize not}\over =}
\def\notaequiv{\buildrel\hbox{\scriptsize not}\over \equiv}
\def\d=f{\buildrel\hbox{\scriptsize d\'{e}f}\over \Longleftrightarrow}


%\def\sec{\stepcounter{subsection}\paragraph{\thesubsection .}}
\def\sec{\stepcounter{subsection}\vskip 18pt
\noindent{\large\bf{\thesubsection}}\hskip 6mm}  

\def\gto{\mathop{\to}\limits_>}


%

\def\cit{\text{\it I\hskip -6ptC\/}}
\def\ptcit{\hbox{${\scriptstyle I\hskip -4ptC\/}$}}
\def\ptrit{\hbox{${\scriptstyle I\hskip -3pt  R\/}$}}
\def\ptnit{\hbox{${\scriptstyle I\hskip -3pt  N\/}$}}
\def\pptcit{\hbox{${\scriptscriptstyle I\hskip -4ptC\/}$}}
\def\pptrit{\hbox{${\scriptscriptstyle I\hskip -3pt  R\/}$}}


\def\square{\hfill\hbox{\vrule height .9ex width .8ex depth -.1ex}}
\def\rit{\text{\it I\hskip -2pt  R}}
\def\dit{\text{\it I\hskip -2pt  D}}
\def\lit{\text{\it I\hskip -2pt  L}}
\def\eit{\text{\it I\hskip -2pt  E}}
\def\Pit{\text{\it I\hskip -2pt  P}}
\def\kit{\text{\it I\hskip -2pt  K}}
\def\zit{\text{\it Z\hskip -4pt  Z}}
\def\qit{\text{\it I\hskip -5.5pt  Q}}
%\def\cit{\hbox{\it I\hskip-7ptC\/}}
\def\nrm{\text{I\hskip -2pt \rm N}}
\def\nit{\text{\it I\hskip -2pt  N}}
\def\rlp {\rit^{\hskip 1pt\ell}_+}
\def\rl {\rit^{\hskip 1pt\ell}}
\def\cip{\hbox{$\cap$ \hskip -8pt $\mid$}}

\def\As{{\cal A}}
\def\Ad{{\text A}}
\def\Bd{{\text B}}
\def\Bs{{\cal B}}
\def\Cs{{\cal C}}
\def\Ds{{\cal D}}
\def\Ed{{\text E}}
\def\Es{{\cal E}}
\def\Fd{{\text F}}
\def\Fs{{\cal F}}
\def\Gd{{\text G}}
\def\Gs{{\cal G}}
\def\Hd{{\text H}}
\def\Hs{{\cal H}}
\def\Id{{\text{\bf I}}}
\def\Is{{\cal I}}
\def\Js{{\cal J}}
\def\Ks{{\cal K}}
\def\Kd{{\rm K}}
\def\Ls{{\cal L}}
\def\Ms{{\cal M}}
\def\Ns{{\cal N}}
\def\Nd{{\text N}}
\def\Os{{\cal O}}
\def\Od{{\text O}}
\def\Ps{{\cal P}}
\def\Pd{{\text P}}
\def\Qs{{\cal Q}}
\def\Qd{{\text Q}}
\def\Rs{{\cal R}}
\def\Ss{{\cal S}}
\def\Sd{{\text S}}
\def\Ts{{\cal T}}
\def\Us{{\cal U}}
\def\Ud{{\text U}}
\def\Xd{{\textstyle X}}
\def\Xs{{\cal X}}
\def\Ys{{\cal Y}}
\def\Zs{{\cal Z}}
\def\Vs{{\cal V}}
\def\Ws{{\cal W}}
\def\rg{\hbox {\sl R}}

\def\nexists{\hbox{$\exists$ \hskip -9pt $\big /$}}

\def\ung{\hbox{1\hskip -4.2pt \rm 1}}
\def \feq {\buildrel \text {def} \over =}

\def \rbar {\rm{R} \hskip-6pt /}
%

\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\beqn{\begin{eqnarray}}
\def\eeqn{\end{eqnarray}}
\def\nobeqn{\begin{eqnarray*}}
\def\noeeqn{\end{eqnarray*}}
\def\ba{\left(\begin{array}}
\def\ea{\end{array} \right) }

\newcommand{\mat}[1]{\left[ \begin{array}{cc}#1
\end{array} \right] }


\def\bpr{\paragraph{Proof.}}
\def\bpre{\paragraph{Preuve} : \hspace{5mm}}
%pour fin de preuve dans paragraphe :
\def\epr{\square\vskip 6pt}
%pour fin de preuve dans équation :
\def\eop{\hbox{\vrule height .9ex width .8ex depth -.1ex}}


\def\u{\underline}
\def\o{\overline}
\def\and{\; \mbox{and} \;}
\def\et{\mbox{\ et\ }}

\def\untilde#1{\mathop{#1}\limits_{\sim}}

\newcommand{\half}{\frac{1}{2}}


\newcommand{\id}{\mbox{} \\ \nopagebreak\vspace{-1cm}}

\def\diagram#1{\def\normalbaselines{\baselineskip=0pt
\lineskip=10pt \lineskiplimit=1pt} \matrix{#1}}

\def\hfl#1#2{\smash{\mathop{\hbox to 12mm{\rightarrowfill}}
\limits^{\scriptstyle #1}_{\scriptstyle #2}}}

\def\vfl#1#2{\llap{$\scriptstyle #1$}\left\downarrow
\vbox to 6mm{}\right. \rlap{$\scriptstyle #2$}}

\def\vupfl#1#2{\llap{$\scriptstyle #1$}\left\uparrow
\vbox to 6mm{}\right. \rlap{$\scriptstyle #2$}}

\def\tg{\mathop{\rm tg}\nolimits}
\def\Th{\mathop{\rm th}\nolimits}
\def\argsh{\mathop{\rm argsh}\nolimits}
\def\argch{\mathop{\rm argch}\nolimits}
\def\argth{\mathop{\rm argth}\nolimits}
\def\argcoth{\mathop{\rm argcoth}\nolimits}
\def\cotg{\mathop{\rm cotg}\nolimits}
\def\ctg{\mathop{\rm ctg}\nolimits}
\def\arcsin{\mathop{\rm arc\ sin}\nolimits}
\def\arccos{\mathop{\rm arc\ cos}\nolimits}
\def\arctg{\mathop{\rm arc\ tg}\nolimits}
\def\Sec{\mathop{\rm sec}\nolimits}
\def\cosec{\mathop{\rm cosec}\nolimits}
\def\arccotg{\mathop{\rm arc\ cotg}\nolimits}
\def\Max{\mathop{\rm Max}}
\def\Min{\mathop{\rm Min}}
\def\minmax{\mathop{\rm min\ max}}

\def\Ker{\mathop{\rm Ker}\nolimits}
\def\Var{\mathop{\rm Var}\nolimits}
\def\cov{\mathop{\rm cov}\nolimits}
\def\argmin{\mathop{\rm argmin}\nolimits}
\def\diag{\mathop{\rm diag}\nolimits}
\def\rank{\mathop{\rm rank}\nolimits}
\def\sgn{\mathop{\rm sgn}\nolimits}
\def\mod{\mathop{\rm mod}\nolimits}
\def\dom{\mathop{\rm dom}\nolimits}


\def\im{\mathop{\rm Im}\nolimits}


\def\sh{\mathop{\rm sh}\nolimits}
\def\ch{\mathop{\rm ch}\nolimits}

\def\Be{\begin{enumerate}}
\def\Ee{\end{enumerate}}

\def\Bena{\begin{enumerate}
\def\labelenumi{\theenumi)}
\def\theenumi{\arabic{enumi}}
\def\labelenumii{\theenumii)}
\def\theenumii{\alph{enumii}}}

\def\Bean{\begin{enumerate}
\def\labelenumii{\theenumii)}
\def\theenumii{\arabic{enumii}}
\def\labelenumi{\theenumi)}
\def\theenumi{\alph{enumi}}}

\def\Bero{\begin{enumerate}
\def\labelenumii{\theenumii)}
\def\theenumii{\arabic{enumii}}
\def\labelenumi{(\theenumi)}
\def\theenumi{\roman{enumi}}}


\def\BeRo{\begin{enumerate}
\def\labelenumii{\theenumii)}
\def\theenumii{\arabic{enumii}}
\def\labelenumi{(\theenumi)}
\def\theenumi{\Roman{enumi}}}



\def\Bi{\vskip 11pt\begin{itemize}\itemsep=18pt}%\topsep=18pt\itemsep=18pt\partopsep=18pt\parsep=18pt}
\def\Ei{\end{itemize}\vskip 11pt}

\def\Bd{\begin{description}}
\def\Ed{\end{description}}

\def\R{\right}
\def\L{\left}
\def\F{\frac}
\def\H{\hat}
\def\T{\tilde}

\newcommand{\photoMatheux}[2]{
\parbox[b][7cm][b]{4cm}{
\epsfig{file=#1,width=3.7cm}
\par\noindent\centerline{{\em #2}}\par\vskip6mm
}}

\newcommand{\GphotoMatheux}[2]{
\parbox[c][11cm][c]{7cm}{
\epsfig{file=#1,width=6.7cm}
\par\noindent\centerline{{\em #2}}\par\vskip6mm
}}


